The Spinning Blimp: Design and Control of a Novel Minimalist Aerial Vehicle Leveraging Rotational Dynamics and Locomotion

This paper presents the Spinning Blimp, a novel lighter-than-air (LTA) aerial vehicle designed for low-energy stable flight. Utilizing an oblate spheroid helium balloon for buoyancy, the vehicle achieves minimal energy consumption while maintaining prolonged airborne states. The unique and low-cost design employs a passively arranged wing coupled with a propeller to induce a spinning behavior, providing inherent pendulum-like stabilization. We propose a control strategy that takes advantage of the continuous revolving nature of the spinning blimp to control translational motion. The cost-effectiveness of the vehicle makes it highly suitable for a variety of applications, such as patrolling, localization, air and turbulence monitoring, and domestic surveillance. Experimental evaluations affirm the design's efficacy and underscore its potential as a versatile and economically viable solution for aerial applications.

==> notincluded.tex <==



%what was the mean and sd for each wing%

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{1.0\linewidth}
%     \includegraphics[width=1.0\linewidth]{figures/error_figure_globalTrack40.png}
%     \caption{Cartesian errors $xyz$.}
%     \end{subfigure}
%     %
%     \begin{subfigure}{1.0\linewidth}
%         \includegraphics[width=1.0\linewidth]{figures/xy_figure_globalTrack40.png}
%     \caption{Plot xy}
%     \label{fig:helix_b}
%     \end{subfigure}
%     %
%     \caption{Lissajous curve caption \fixme{Grid, and mean dev etc should go in the paragraph}}
%     \label{fig:helix}
%     \vspace{-1em}
% \end{figure}
    %\subsubsection{{Endurance Experiment}}
    %\subsubsection{Turning Left vs Turning Right}
    %Highlight from the figure 
    %\subsubsection{Random walk}
    

    %%%%%%%%%%% Place velocity chart here
   %  \begin{figure*}[t]
   %  \centering
   %  \setlength\fboxsep{0pt}
   %  \setlength\fboxrule{0.25pt}
   %      \minipage{0.32\textwidth}
   %        \includegraphics[width=\linewidth]{figures/error_figure.png}
   %        \caption{}\label{fig:awesome_image1}
   %      \endminipage\hfill
   %      \minipage{0.32\textwidth}
   %        \includegraphics[width=\linewidth]{figures/error_figure.png}
   %        \caption{}\label{fig:awesome_image2}
   %      \endminipage\hfill
   %      \minipage{0.32\textwidth}%
   %        \includegraphics[width=\linewidth]{figures/error_figure_lissajous.png}
   %        \caption{Case 3}\label{fig:awesome_image3}
   %      \endminipage
    
   %  % \caption{Bang bang control for trajectory of Spinning Blimp with respect to reference position along circle}
   %  \label{f7}
   %  \end{figure*}

   % \begin{figure*}[t]
   %  \centering
   %  \setlength\fboxsep{0pt}
   %  \setlength\fboxrule{0.25pt}
   %      \minipage{0.32\textwidth}
   %        \includegraphics[width=\linewidth]{figures/x_vs_y_plot.png}
   %        \caption{}\label{fig:awesome_image1}
   %      \endminipage\hfill
   %      \minipage{0.32\textwidth}
   %        \includegraphics[width=\linewidth]{figures/x_vs_y_plot.png}
   %        \caption{}\label{fig:awesome_image2}
   %      \endminipage\hfill
   %      \minipage{0.32\textwidth}%
   %        \includegraphics[width=\linewidth]{figures/x_vs_y_plot_lissajous.png}
   %        \caption{Case 3}\label{fig:awesome_image3}
   %      \endminipage
   %      \caption{9: x-y-z position data from reference circle tracking, 10: x-y position, 11: x-y-z position data from reference Lissajous Curve, 12: x-y position. Bang bang control for trajectory of Spinning Blimp with respect to reference position along circle}
   %  \label{f7}
   %  \end{figure*}
    
    % \item Light Following Test: 
    % \item Lissajous Circle Tracking Test: 

% \qbleo{combine xyz error}

% \begin{figure*}[t]
%     \centering
%      \includegraphics[width=1.0\textwidth]{figures/PlotC.jpg}
%       \caption{Experiment Tracking}
%        \label{fig:mainrobot}
% \end{figure*}




% {\footnotesize
% \begin{eqnarray*} 
% \label{eq1}
%         \begin{bmatrix}
%         p \\ q \\ r\\ \end{bmatrix}
%         &=& \begin{bmatrix}
%             \cos{\psi} & -sin{\psi} & 0\\
%             \sin{\psi} & cos{\psi} & 0\\
%             0 & 0 & 1\\\end{bmatrix}
%         \begin{bmatrix}
%         \dot{\theta} \\ \dot{\phi} \\ \dot{\psi}\\ \end{bmatrix}\\
%         I 
%         \begin{bmatrix}
%             \dot{p} \\ \dot{q} \\ \dot{r}\\ \end{bmatrix}
%         &=&
%         \begin{bmatrix}
%         r_{m}(F_{1}-F_{2}) \\ r_{m}(F_{1}-F_{2}) \\ r_{m}(F_{1}+F_{2}) \end{bmatrix}
%         - 
%         \begin{bmatrix}
%         p \\ q \\ r\\ \end{bmatrix} \times I 
%         \begin{bmatrix}
%         p \\ q \\ r\\ \end{bmatrix}\\
% \end{eqnarray*}
% }
\newpage
.
\newpage

\section{Appendix A}

\captionof{table}{MAV Flight Characteristics}  
\begin{tabular}{ |p{1.2cm}||p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|  }
 \hline
 \multicolumn{5}{|c|}{MAVs List \cite{10.3844/ajeassp.2022.316.330}} \\
 \hline
 MAV's Name or Institution Name& Battery Size (mAh)& Total Mass (g) &Claimed Flight Endurance (min) & Vol. Helium ($m^3$)\\
 \hline
 GT-MAB          && 0 & 120&\\
 S-Cloud         && 60 & 63 &\\
 S-Cloud II      && 50-100& 120&\\
 SpICED Blimp    && 0 & ?&0.2681\\
 ModBlimp        &&&&\\
 NMIMT           & 1300& 214.9 & 48&\\
 Skye            && ?& 120& 10.31\\
 Plantraco       && 0 &?&\\
 \hline

\end{tabular}

\section{Appendix B}
{\footnotesize
To linearize the given system of equations, we need to find the linear approximation of each equation around a specific operating point. Linearization involves taking the first-order Taylor series expansion of each equation with respect to the variables involved. This process assumes that the deviations from the operating point are small, so only the first-order terms are considered.

Given system of equations:
\[
\begin{bmatrix}
\Delta xy \\
\Delta z \\
\end{bmatrix}
=
\begin{bmatrix}
|F_{xy,des}| \Bigl(\sin(\theta_{xy})\cos(\psi) + \cos(\theta_{xy})\sin(\psi) \Bigr) - K_{D}v_{xy}^2 \\
2k_F\dot{\psi}^2 + f_{b} - mg \\
\end{bmatrix}
\]

I assumed an operating point at $\theta_{xy} = \theta_{xy_0}$ and $\psi = \psi_0$, and $v_{xy} = v_{xy_0}$ and $\dot{\psi} = \dot{\psi}_0$.


1. For $\Delta xy$ equation:
\begin{eqnarray*}
\frac{\partial \Delta xy}{\partial \theta_{xy}} &= |F_{xy,des}| \Bigl(\cos(\theta_{xy_0})\cos(\psi_0) - \sin(\theta_{xy_0})\sin(\psi_0) \Bigr) \\
\frac{\partial \Delta xy}{\partial \psi} &= |F_{xy,des}| \Bigl(-\sin(\theta_{xy_0})\sin(\psi_0) + \cos(\theta_{xy_0})\cos(\psi_0) \Bigr) \\
\frac{\partial \Delta xy}{\partial v_{xy}} &= -2K_Dv_{xy_0}
\end{eqnarray*}

2. For $\Delta z$ equation:
\[\frac{\partial \Delta z}{\partial \dot{\psi}} = 4k_F\dot{\psi}_0\]
(Note: There is no $\theta_{xy}$ term, so its derivative is zero.)

\begin{eqnarray*}
\Delta xy &\approx \frac{\partial \Delta xy}{\partial \theta_{xy}} \Bigg|_{\theta_{xy} = \theta_{xy_0}, \psi = \psi_0, v_{xy} = v_{xy_0}} \cdot (\theta_{xy} - \theta_{xy_0}) \\
&\quad + \frac{\partial \Delta xy}{\partial \psi} \Bigg|_{\theta_{xy} = \theta_{xy_0}, \psi = \psi_0, v_{xy} = v_{xy_0}} \cdot (\psi - \psi_0) \\
&\quad + \frac{\partial \Delta xy}{\partial v_{xy}} \Bigg|_{\theta_{xy} = \theta_{xy_0}, \psi = \psi_0, v_{xy} = v_{xy_0}} \cdot (v_{xy} - v_{xy_0})
\end{eqnarray*}

\begin{eqnarray*} \Delta z \approx \frac{\partial \Delta z}{\partial \dot{\psi}} \Bigg|_{\dot{\psi} = \dot{\psi}_0} \cdot (\dot{\psi} - \dot{\psi}_0)
\end{eqnarray*}

This linearization is only valid in a small neighborhood around the operating point, where the deviations from the operating point values are small. This follows our assumption of the attitude changes of Spinning Blimp being zero.


\begin{eqnarray*}
\Delta xy &\approx& \frac{\partial \Delta xy}{\partial \theta_{xy}} \Bigg|_{\theta_{xy} = \theta_{xy_0}} \cdot (\theta_{xy} - \theta_{xy_0}) 
+ \frac{\partial \Delta xy}{\partial \psi} \Bigg|_{\psi = \psi_0} \cdot (\psi - \psi_0) \\
+ \frac{\partial \Delta xy}{\partial v_{xy}} \Bigg|_{v_{xy} = v_{xy_0}} \cdot (v_{xy} - v_{xy_0})\\
\Delta z &\approx& \frac{\partial \Delta z}{\partial \dot{\psi}} \Bigg|_{\dot{\psi} = \dot{\psi}_0} \cdot (\dot{\psi} - \dot{\psi}_0)\\
\Delta xy &\approx& |F_{xy,des}| \left(\cos(\psi_0)(\theta_{xy} - \theta_{xy_0})
- \sin(\psi_0)(\psi - \psi_0)\right) - 2K_Dv_{xy_0}(v_{xy} - v_{xy_0})\\
\Delta z &\approx& 4k_F\dot{\psi}_0 \cdot (\dot{\psi} - \dot{\psi}_0)
\end{eqnarray*}

}


\section{Intro}
\david{
\todo{what is the purpose of this paragraph?}
\todo{I wanted to cite other helium assisted vehicles. I think I need to define what differentiates our approach of using helium balloons to the others}
In the search of MAVs for studying swarm behaviours and under-actuated designs, many researchers have settled on helium assisted vehicles. More recently, be-it using direct drive actuators or aerodynamic Coanda effects, combining MAVs with helium balloons increases human interaction safety in the lab, longer flight times, higher payloads and natural stability. Building upon the ground covered by GT-MAB, S-CLoud, Skye, SpICED \cite{song_design_2020, burri_design_2013, seguin_deep_2020, hodgson_precision_2016, hwan_song_design_2018, wan_design_2018, cho_autopilot_2017, gonzalez_developing_2009, lonneville_helium_2014} and more, has brought interest in our lab to combine natural spinning behaviours and helium assisted MAV designs together.
}




% Using a single wing and single actuator, the nature inspired Samara wing \cite{ulrich_control_2010} as well as a semi-rigid foldable Samara wing F-SAM \cite{win_design_2021} utilize cyclic control. 
% Dual actuated example stem from the original bicopter design \cite{gress_using_2002} but have also taken inspiration from natural autorating behaviours such as a dual actuated spinning samara \cite{bai_bioinspired_2022}\cite{9882300} and a flapping winged mechanism \cite{ma_controlled_2013}.
%Further complexities such as tricopters \cite{rongier_kinematic_2005}\cite{salazar-cruz_stabilization_2009} and quadcopter designs \cite{pounds_design_2002} showcase higher capabilities for controllable degrees of freedom. However, for surveying purposes, random walk behaviours and swarm behaviours more complex systems present a question whether less degrees of free are capable of the same tasks.
%Continuous mapping using multirotors \cite{kaul_continuous-time_2016} and self-rotating MAVs \cite{chen_self-rotating_2023} set the stage for finding solutions or behaviours that inherently accomplish the tasks.

% Two wings - two motors \cite{gress_using_2002}
% nus spinning bicopter \cite{bai_bioinspired_2022} flapping two wing 
% Tricopter
% original tricopter \cite{rongier_kinematic_2005} , tailrotor tricpoter \cite{salazar-cruz_stabilization_2009}
% Quadcopter
% original quadcopter \cite{pounds_design_2002}

% spinning mapping
% Continuous mapping \cite{kaul_continuous-time_2016} Self-rotating \cite{chen_self-rotating_2023}

% Paper's that make use of helium balloons


% Check for overlap in related works creates the gap that we define

% Discuss the combination of spinning with balloons Pro/Con

The purpose of creating a minimalistic aerial vehicle is two fold. Firstly, reducing the components combined with a novel control strategy simplifies the understanding of the vehicle for educational purposes. Secondly, minimizing the number of intricate components parts helps create a low barrier-to-entry for utilization in collaborative environments (e.g. swarms).
% \subsection{Advantages over other robots}

\subsection{Contribution}
An aerial vehicle combining a helium balloon and a two bladed wing reduces the complexity of the system. The minimalistic design of reducing a multi-rotor with n-actuators and six degrees of freedom to a system with two actuators and three degrees of freedom. The simplified actuation takes advantage of a passive lifting mechanism to control lift.

% no reliance on attitude controller
The under-actuated design creates a limitation for controlling attitude. However, to be explained later, the natural buoyancy couple ensures the attitude controller is not a necessary condition for controlled flight.




The minimalistic requirement for controlled flight helps reduce the cost of producing the vehicle. Through the benefit of a helium balloon, the lowered lifting requirement means spinning blimp can take advantage of large slow revolving wings. This results in smaller motors and small propellers being required.

% minimalistic sensing requirement
The inherent spinning behaviour produces a reduced complexity for sensing requirement. LiDAR, a remote sensing method measured using Time of Flight (ToF) laser sensors, requires a motor to rotate a laser's reflective mirror to completely sense the 360$^{
\circ}$ surroundings of a robot. Utilizing the spinning behaviour means the ToF sensor is inherently spinning at Spinning Blimp's angular velocity.

% simplified actuation
The single degree-of-freedom actuation based on a cycle average approach reduces the complexity of position control. Utilizing the passive attitude stability, later to be shown, allows Spinning Blimp to solely focus on position control in the global reference frame XYZ through modulating two motor forces.

% economical design (low-cost) (less wearing components)
Compared to a multi-rotor or a swash plate design of a helicopter, Spinninng Blimp reduces the number of wearing components to two motors and a lithium-ion polymer battery (LiPo).


% claims can come  from this area (introduce claims that are in experiments)

As the space of micro aerial vehicles (MAVs) becomes increasingly more complex and researched, MAVs require multiple more components to achieve stable flight conditions. Spinning Blimp achieves global passive stability, increase flight endurance over comparable helium assisted lighter than air vehicles and is more economical to manufacture.

% Narrowing down the scope (each successive describe point narrows down the challenge)
% Describe challenge of stability


% Describe challenge of flight time
The space of aerial robotics consistently faces challenges of creating platforms with long endurance. The balance comes from creating a lightweight system or adding more energy storage at the cost of weight. As show in the state of the art \cite{bai2022}, high disk loading MAVs quickly reach flight endurance limits. Overcoming flight endurance challenges allows MAVs to focus on mission capabilities.
% Helium is one of the most abundant resources in the universe, and once helium is released into the atmosphere, it can easily escape and be released into space. 
Although adding helium reduces the impact of inefficient aerial mobility, utilizing momentum theory to create efficient flight helps reduce the reliance on helium.



% Describe challenge of sensing


% Main contribution this paper provides (layout for reviewer explicity)

% human safe design
% Application
\subsection{Use cases}
Since our Spinning Blimp can work with short wings(less radius than the helium balloon), the contact area of the robot will be the soft balloon part, which means it's will bounce when impact occurs while moving. It's safe to most objects in the environment, including human. This feature gives it the ability to work with human without any extra protection, such as doing exploration moving with human, or carrying payload following human. Besides, the Spinning Blimp can carry a camera and work as a monitor of a certain area with animals or humans, which is powered by the long flight time, inherent spinning behaviour, and safety of our robot. Another example of application is autonomous warehouse stock inventory, which also needs a robot with long working time, safe to the environment, and a wide range of sensing.




\section{Old design}


    The relationship between drag ($D$) and the square of the radius ($r^2$) is due to the drag force's dependence on the object's cross-sectional area ($A \sim r^2$) in the drag equation $D = \frac{1}{2} 
    C_d\rho AV^2$. Conversely, lift ($L$) is related to the cube of the radius ($r^3$) because the pressure difference contributing to lift is influenced by the object's curvature and shape, with pressure changes proportional to the cube of the radius ($\Delta P \sim r^3$) in the lift force equation $L = \Delta PA$. Thus, allowing Spinning blimp to adapt the buoyant force requirements with minimal drag impact. 



\begin{enumerate}


    \item Propeller Configuration: mounted in proximity to the wings are two small propellers. Configurations in arm length from the center of mass investigates momentum and inertial trade-offs for varying arm from axis of rotation. The propeller configuration is denoted by rotation matrix $\!\boldsymbol{R(\alpha)}\!_x$ highlighting the contribution of the motor forces to a body frame axis other than y. This design is chosen to maximize translational contribution of the small brushed motors. With majority of height being compensated by a light than air gas, the final design focused on investigating lift solely being generated by the wing.

    \item Wing Span: two wing configuration of 0.7m and 1.3m diameter wings were created. The affects this creates is described in Blade Element Momentum Theory (BEMT) for a propeller, where $dL$ represents the incremental change in lift, while $dD$ represents the incremental change in drag for a small section of a propeller blade. As the propeller's diameter increases, $dL$ and $dD$ grow due to the greater radial distance from the hub to the blade section ($r$), resulting in higher linear velocities ($v$) and consequently increased lift and drag \cite{driessens_triangular_2015,sammut_australasian_2005}. In the realm of propeller dynamics, the blade element momentum theory is a pivotal concept in understanding propulsion efficiency. Imagine contrasting scenarios: a propeller with a large diameter (L) rotating at a slower speed and another with a smaller diameter (S) rotating at a higher speed. Both propellers generate equal thrust (T) and rotate at the same RPM (N). The power needed to sustain this thrust can be defined as the product of thrust and velocity:
    
    \[ P = T V. \]
    
    The blade element theory provides a formula for the thrust produced by a minuscule blade segment: \(dT = 2\pi r \cdot \rho \cdot A \cdot v \cdot \delta v\). In this equation, \(r\) signifies the radial distance, \(\rho\) stands for air density, \(A\) represents the blade area, \(v\) denotes velocity, and \(\delta v\) corresponds to the velocity differential across the blade segment.
    
    The crucial aspect lies in the quadratic relationship between velocity and kinetic energy: \(KE = \frac{1}{2} m v^2\). As velocity increases, kinetic energy grows quadratically, and subsequently, so does the energy needed to produce thrust. In the case of the smaller propeller (S), the higher velocity translates to a more substantial velocity differential (\(\delta V\)) across the blade segment compared to the larger propeller (L). This engenders a quadratic rise in induced drag, leading to diminished efficiency for the smaller propeller. Mathematically:
    
    \[dT_{S} = 2\pi r \cdot \rho \cdot A_{S} \cdot v \cdot \delta v_{S} \quad \text{and} \quad dT_{L} = 2\pi r \cdot \rho \cdot A_{L} \cdot v \cdot \delta v_{L},\]
    
    where \(\delta V_{S} > \delta V_{L}\), resulting in \(dT_{S} > dT_{L}\). In essence, the quadratic relationship between velocity and energy expenditure accentuates the inefficiency of the smaller, faster-moving propeller when compared to the larger, slower-moving counterpart \cite{prouty_helicopter_1995}.
    \item Frame: Foam core cut using a $CO_{2}$ laser cutter. The combination of lightweight foam for strength and paper lining ensures rigidity should foam crack.
    % The equations for $dL$ and $dD$ are given by:
    % \begin{align*}
    % dL &= 2\pi \cdot r \cdot dr \cdot \alpha \cdot c_l \cdot \rho \cdot v^2 \\
    % dD &= 2\pi \cdot r \cdot dr \cdot c_d \cdot \rho \cdot v^2
    % \end{align*}
    % Here, $r$ is the radial distance from the hub to the section, $dr$ is the differential radial thickness, $\alpha$ is the local angle of attack, $c_l$ is the coefficient of lift for the airfoil section, $c_d$ is the coefficient of drag for the airfoil section, $\rho$ is the air density, and $v$ is the linear velocity.    
\end{enumerate}


\section{Old Model}


%Propeller dynamics are expressed using lumped mass assumptions. 
% Thereby allowing the consolidation of small motor forces represented as $f_{i}$.
Where $f_{i} = f_{h}\pm  \tau$. $f_{h}$ represents the forces required to sustain hover and differential thrust force $\tau$ represents the translational forces. 

The point at which the motor act along Spinning Blimp's body frame x-axis is represented as $p_{m}$.

% The buoyant force explored is $f_{b}$ and this force acts at point and is represented by the vectorized point $\boldsymbol{p_{b}}$. The buoyant force,         $f_{b} = \rho V g$ 
% is comprised of the density $\rho$, volume displaced $V$ and acceleration due to gravity on the volume displaced $g$. 

%The coordinate frames require rotation matrices from the body reference frame to the world frame .
The planar disk attitude of the spinning blimp is referenced to the fixed reference frame with global coordinates $x \And y$. $\theta$ and $\phi$ denote angles around the $x \And y$ axis respectively and $\psi$ denotes yaw around the $z$-axis. The robot has a reference point located in the Center of Mass (CoM). This point is denoted by the black and white CoM symbol. 





Spinning Blimp depends on the relationship between the angular velocity $\boldsymbol{\omega}$ to produce the required lifting forces from the two winged surfaces. Where $\boldsymbol{\omega}$ is a vector of angular velocities in $x, y$ and $z$ of the body reference frame. The lift dynamics are denoted by the coefficient $k_{lift}$ and surface area s.

The drag produced by Spinning Blimp's wings are denoted by a diagonalized coefficient $\boldsymbol{K_{d}}$ and for Spinning Blimp the assumption is present that drag is dependent on the quadratic of the linear velocity in the three coordinate axes.



By transforming the forces from the body frame to the world frame, we obtain
% The lift force produced by the winged surfaces is denoted in the body frame and requires a rotation matrix. Lastly, the drag produced by the wing is denoted by the linear velocity in the body frame.
% {\footnotesize
\begin{eqnarray*} 
        m
        \ddot{\boldsymbol{x}}
        &=&
        {}^W\!\!\boldsymbol{R}\!_B . \!\!\boldsymbol{R}\!_x(\alpha)
        \begin{bmatrix}
        0\\ \sum_{i=1}^{2} f_{i}\\ 0 \end{bmatrix}
        + 
        \begin{bmatrix}
        0\\ 0\\ -mg + f_{b} \end{bmatrix}
        \\
        %
        &+&
        {}^W\!\!\boldsymbol{R}\!_B
        \begin{bmatrix}
        0\\ 0\\ k_{lift} s {\omega_z^2} \end{bmatrix}
        + 
        {}^W\!\!\boldsymbol{R}\!_B \boldsymbol{K_{d}}
        \begin{bmatrix}
        v_x|v_x|\\ v_y|v_y|\\ v_z|v_z|\\
        \end{bmatrix}
        \label{eq:newton2}
\end{eqnarray*}

\begin{eqnarray*}
%{}^W\!\!\boldsymbol{R}\!_{B,x} = \begin{bmatrix}
%            \cos{\theta} & 0 & sin{\theta}\\
%            0 & 1 & 0\\
%            -\sin{\theta} & 0 & %\cos{\theta}\\\end{bmatrix}  
%            \\
%{}^W\!\!\boldsymbol{R}\!_{B,y} = \begin{bmatrix}
%            1 & 0 & 0\\
%            0 & \cos{\phi} & -sin{\phi}\\
%            0 & \sin{\phi} & cos{\phi}\\
%            \end{bmatrix} 
%            \\
\!\boldsymbol{R}(\alpha)\!_x &=& \begin{bmatrix}
            1 & 0 & 0\\
            0 & \cos{\alpha} & -\sin{\alpha}\\
            0 & \sin{\alpha} & \cos{\alpha}\\
            \end{bmatrix}\\
\!\boldsymbol{R}(\psi)\!_z &=& \begin{bmatrix}
            \cos{\psi} & -\sin{\psi} & 0\\
            \sin{\psi} & \cos{\psi} & 0\\
            0 & 0 & 1\\\end{bmatrix}.\\
\end{eqnarray*}



The representation of stabilizing buoyant forces is represented by the rotation from world to body frame matrix and the torque created by the buoyant couple about the center of pressure $p_{b}$  (figure \ref{fig:coordinates}). $p_{W}$ represents the quadratic drag generated by the angular velocity of the wings. This is represented in equation \ref{eqn7}

\begin{eqnarray*}
    \boldsymbol{I} \boldsymbol{\dot{\omega}} =\sum_{i=1}^{2} p_{i,m} \times \!\boldsymbol{R}\!_x(\alpha)
    \begin{bmatrix}
    0\\ \sum_{i=1}^{2} f_{i}\\ 0 \end{bmatrix}&
    \\
    + 
    p_{b} \times {}^B\!\!\boldsymbol{R}\!_W \begin{bmatrix} 0\\ 0\\ f_{b} \end{bmatrix}
    + p_{W}
    \begin{bmatrix} 0\\ 0\\ k_{w} s  \omega^2 \end{bmatrix} - \omega \times \boldsymbol{I}\omega. 
\end{eqnarray*}




\section{old discussion}

\subsection{DC Motor}




As seen in the existing control policy, for directional control, $\psi$ is used to apply sinusoidal control curves. The non-linear actuation produced by brushed DC motors prompted investigation into methods of control with lower actuation delays and losses. The motor outputs, for control in the x-direction of the body reference frame, can be defined as follows:

\subsection{Helium}
In the research community the benefit of helium-assisted vehicles has been presented. However, the case to be made is varying the volume to accommodate a larger battery can produce varying results in flight endurance. The case to be made is how does comparing equal volume and equal battery exemplify the performance of Spinning Blimp.

\subsection{Random walk}



\subsection{Simulation}
% In this section, implementation and results of a simulated drag forces and tracking are presented.
% \subsubsection{Simulation Setup}
The goal of simulation is to evaluate the model and control algorithm, as well as generating a result as a reference of real world experiment.  We designed and implemented the simulation based on Pylab in JupyterNotebook. Before we run the simulator, we need to set up the configuration of the robot and environment, such as size of the robot, weight, motor position, inertia, initial state, also the dynamic and control policy. Then the simulator will run step by step in certain amount of time and interval, generate log file of states of the robot and plot the result, and come up with an animation video. We had tested PD position controller, PD velocity controller and bang-bang control input, under the simulation of square way-points, circle position tracking and Lissajous position tracking. 

% Momentum effects of movement close to walls showed results the need for detection that Spinning Blimp had indeed moved away from a wall. Should Spinning Blimp not be able to escape a confined space, by seeing another wall that would fixate its position, a period of 6 seconds is put in place where no direction change is allowed. Following this period a random direction change inside a window of $-25 < \theta > 25$ from the direction movement is added to force movement in rectangular environments. 
% The greatest limitation with the VL53L1X ToF sensor is a detection only occurs within 2.5 meters.   

%%% Discussion points %%%%
\subsubsection{Turning Left versus Right}



\subsubsection{Wind resistance}




\subsection{Passive position stability}
The larger wing, during a robotics research competition was able to stay aloft and remain in position with minimal control input. To accommodate the same research platform for comparison the same materials were use to construct each robot. Be it through dihedral affects of bending wings during turbulence, larger inertial properties or a large tip path plane, the larger wing span provides more resilience than the smaller wing for inherent position stability.

\subsection{Angle of Blades affects angular velocity}

% \subsubsection{Resilience to wing fracture}


% \newpage
% .
% \newpage

\section{Behaviours}

% \subsection{Differential Light Following - Braitenberg Vehicle}
% \subsection{Random Walk}


% \newpage
% .
% \newpage


spinning robots
\cite{bai2022} \cite{chen2023} \cite{Win2021}

